Assessing the Reliability of Visual Explanations of Deep Models with Adversarial Perturbations

The interest in complex deep neural networks for computer vision applications is increasing. This leads to the need for improving the interpretable capabilities of these models. Recent explanation methods present visualizations of the relevance of pixels from input images, thus enabling the direct interpretation of properties of the input that lead to a specific output. These methods produce maps of pixel importance, which are commonly evaluated by visual inspection. This means that the effectiveness of an explanation method is assessed based on human expectation instead of actual feature importance. Thus, in this work we propose an objective measure to evaluate the reliability of explanations of deep models. Specifically, our approach is based on changes in the network's outcome resulting from the perturbation of input images in an adversarial way. We present a comparison between widely-known explanation methods using our proposed approach. Finally, we also propose a straightforward application of our approach to clean relevance maps, creating more interpretable maps without any loss in essential explanation (as per our proposed measure).

==> analysis.tex <==
\section{Further Analysis}
\label{sec:analysis}

In this section we discuss some interesting properties of APEM. We expect that these properties could benefit future application scenarios.

\subsection{The Importance of Irrelevance Maps}

As discussed previously, the inverse of relevance is also taken into account while calculating APEM. This is important because it prevents the explanation methods from focusing on a few relevant pixels, while not giving importance to others that may be also relevant. In this sense, considering irrelevance gives the metric a \emph{recall}-like property. %Since APEM is essentially measuring the extent to which all relevant pixels are contained in the relevance map, taking into account relevance and irrelevance information emphasizes the precision$-$recall notion while calculating APEM.
%To illustrate this, consider the following scenarios and the corresponding expected behavior of APEM:

%\begin{itemize}
%\item The relevance map comprises one region as important, while both this region and another one are actually important: in this case $\epsilon^-$ has a low value, but $\epsilon^+$ drastically decreases since there are relevant pixels being considered in its calculation, making the model to misclassify the perturbed image faster. Thus, APEM decreases as a relevant region is not being considered.
%\item The relevance map comprises two regions as important while just one of these regions is actually important: in this case even though $\epsilon^+$ is not penalized because there is no relevant pixel in the irrelevance map, $\epsilon^-$ increases as irrelevant regions are being considered.
%\end{itemize}

In order to investigate the importance of also considering $\epsilon^+$ (irrelevance) when calculating APEM, we compared LRP with  SmoothGrad while only considering irrelevance values. Figure \ref{fig:gap_vs_rel} shows the histogram and the kernel density estimate of the difference between $\epsilon^+$ values from LRP and SmoothGrad. Although LRP presents higher APEM values than SmoothGrad, we observed that LRP produces relevance maps that are often more focused than those produced by SmoothGrad. LRP is, then, penalized for this and has lower $\epsilon^+$ values than SmoothGrad on average -- in this case a lower $\epsilon^+$ results in a reduction in its APEM value.

% Although LRP presents better APEM numbers than SmoothGrad, we observed that LRP produces relevance maps that are often smaller than those produced by SmoothGrad. This behavior may be due to the possibility of observing lower $\epsilon^+$ values even when APEM values are higher. That is, $\epsilon^-$ have contributed to increase APEM. Figure \ref{fig:gap_vs_rel} shows the histogram and the kernel density estimate of the difference between $\epsilon^+$ values from LRP and SmoothGrad, for each image in which $\epsilon^-$ values from LRP are lower than $\epsilon^-$ values from SmoothGrad. This suggests that considering $\epsilon^-$ helps incorporating relevant pixels into the relevance map.

% Although LRP presents better APEM numbers than SmoothGrad, we observed that LRP produces relevance maps that are often smaller than those produced by SmoothGrad. This behavior may be due to the possibility of observing lower $\epsilon^+$ values even when APEM values are higher. That is, $\epsilon^-$ have contributed to increase APEM. Figure \ref{fig:gap_vs_rel} shows the histogram and the kernel density estimate of the difference between $\epsilon^+$ values from LRP and SmoothGrad, for each image in which $\epsilon^-$ values from LRP are lower than $\epsilon^-$ values from SmoothGrad. This suggests that considering $\epsilon^-$ helps incorporating relevant pixels into the relevance map.
%We noticed that the irrelevance of LRP has both greater and lower values than the other one because it also contains relevant pixels in some cases, even if APEM is higher.

\begin{figure}[t]
\centering
\includegraphics[width=.8\linewidth]{img/gap_vs_rel.pdf}
\caption{Histogram and kernel density estimate of the difference between $\epsilon^+$ of LRP and SmoothGrad methods. Positive values are observed when $\epsilon^+$ for LRP is higher than for SmoothGrad, and negative otherwise.}
\label{fig:gap_vs_rel}
\end{figure}

\subsection{Random Relevance Maps}

In order to investigate the robustness of APEM, we use the same $5{,}000$ input images and their respective relevance maps evaluated in Section \ref{sec:results}. However, in this experiment, we shuffled the relevance and irrelevance maps to create random maps based on the same distribution given by the explanation methods. Thus, random relevance maps are supposed to have the same $\epsilon^-$ and $\epsilon^+$, since the relevance values are now high in both truly relevant as well as in non-relevant pixels. For each image, ten shuffled maps were created and if one of them is misclassified, then the values of $\epsilon^-$ and $\epsilon^+$ are retrieved. We tested this at each of the three filtering steps for the Gradient method, and Figure \ref{fig:shuffle_hist} shows the results. Clearly, APEM values concentrate around zero. This is expected, as random relevance maps do not provide actual explanations.
While we show results only for the Gradient method, the same trend was observed for the other explanation methods.

%We also compared average and median APEM values using the same process for all explanation methods. Again,  average oscillates around zero, and the median is zero for every case tested. 

\begin{figure*}[t]
\centering
\includegraphics[width=.9\linewidth]{img/shuffle/shuffle_simple_hist.png}
\caption{Histogram of APEM values for shuffled relevance maps after each filtering step. Relevance maps from the Gradient explanation method. APEM oscillates around zero, meaning that random relevance maps (i.e., bad explanations) will result in APEM values that are close to zero.}
\label{fig:shuffle_hist}
\end{figure*}

%Thus, we may use this shuffling strategy to simply normalize the original APEM values as:
%$$
%\mbox{APEM}_{norm} = \frac{\displaystyle\sum_{i=1}^n{\left( \frac{\epsilon_i^+}{\epsilon\text{-}shuffle_i^+} - \frac{\epsilon_i^-}{\epsilon\text{-}shuffle_i^-} \right)}}{n}
%$$

%Recalculating the results presented in Section \ref{sec:results} with the new normalized $\text{APEM}_{norm}$ results in the values shown in Table \ref{tab:norm_apem}. As $\epsilon\text{-}shuffle^+$ and $\epsilon\text{-}shuffle^-$ are known to be equal or very close, and their values are between the maximum and minimum $\epsilon$, represented by $\epsilon^-$ and $\epsilon^+$, the normalization keeps the same properties of the original APEM but in a space where the values are useful for visualization and comparisons.

%\begin{table}[t]
%    \centering
%    \begin{tabular}{l | c c c}
%        \toprule
%         & 1 & 2 & 3 \\ 
%        \midrule
%         Gradient & \textbf{1.11} & \textbf{0.85} & \textbf{0.66} \\
%         Smooth Grad & 0.39 & 0.30 & 0.21 \\
%         LRP & 0.53 & 0.48 & 0.40 \\ 
%        \bottomrule
%    \end{tabular}
%    \caption{$\text{APEM}_{norm}$ calculated from shuffled relevance maps for each explanation method after each filtering step. The steps are the first 3-channel relevance image (1), the mapping to one channel (2) and the resulting image of the multiplication of this final map with the original input image (3).}
%    \label{tab:norm_apem}
%\end{table}


\subsection{Misclassified Images}

So far our analysis only considered a set of $5{,}000$ correctly classified images. In order to properly explain and debug a model, we also have to understand how APEM behaves with misclassified images. Thus, we performed the same evaluation process on a set of $5{,}000$ misclassified images. In this case, the labels we used to create relevance maps were the ones predicted by the model.

As (hopefully) expected, the model is more uncertain about a decision when it predicts a wrong label. Then, it is expected that the model does not need many perturbations to make it change a prediction, which results in lower $\epsilon$ values. This leads to lower APEM values. On the other hand, this should not influence the quality of the explanation, disregarding the understanding of the generated relevance map. To put it simple, the overall APEM values are decreased but the best explanation methods should to keep their ranking positions.

Table \ref{tab:apem_results_wrong} shows average and median APEM values, comparing them with the ones obtained with the correctly classified images. The APEM decrease is clear, but the relative ordering of the explanation methods remains the same.

\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l rrrr}
        \toprule
        & \multicolumn{2}{c}{Loss} & \multicolumn{2}{c}{Median} \\ \cmidrule(r){2-3} \cmidrule(r){4-5}
         & Correct & Misclassified & Correct & Misclassified \\ 
        \midrule
         Gradient & \textbf{127.79} & \textbf{43.58} & \textbf{81.00} & \textbf{25.00} \\
         Smooth Grad & 44.38 & 12.65 & 16.00 & 4.00 \\
         LRP & 66.07 & 20.34 & 41.00 & 11.00 \\ 
        \bottomrule
    \end{tabular}}
    \caption{Average and Median APEM values for correctly classified and misclassified images. Maps are calculated considering the prediction as the ground truth. Misclassification leads to an overall APEM decrease.}
    \label{tab:apem_results_wrong}
\end{table}

\subsection{Correlation between APEM and Loss}

The last set of experiments is devoted to investigate the possible correlation between APEM and loss. For this, we used the correctly classified images, misclassified images, and the total set of images. Again, the relevance map calculated for the misclassified images is based on the model prediction even though the loss uses the ground truth. The greatest probability for a label in the prediction is referred to as confidence, and it is also compared with the loss.

We compute the correlation using the Spearman's rank correlation coefficient \cite{croux2010influence} because of the non-linear relationships present in the data. This correlation is equal to the Pearson correlation between the rank values of the variables. A correlation close to $+$1 occurs when the observations have a similar rank between the variables, and it is close to $-$1 when they have a dissimilar one.

Table \ref{tab:corr} shows the correlations and the statistical significance. The correlation analysis indicates that correctly classified images have higher correlations while the misclassified images have virtually none. Also, observations have a dissimilar rank between APEM and loss, resulting in a negative correlation. Further, the methods that achieve higher APEM values also are the ones with higher correlation. In summary, the best explanation methods in terms of APEM have a higher correlation with the loss. Finally, high APEM values mean lower losses. Therefore, good explanations given by high APEM values can be used to assess the reliability of the model output.

\begin{table}[t]
    \centering
    \resizebox{0.75\linewidth}{!}{
    \begin{tabular}{l rrr}
        \toprule
        & \multicolumn{3}{c}{Loss} \\ \cmidrule(r){2-4}
         & Correct & Misclassified & Full \\ 
        \midrule
         Gradient & $\text{-}0.827^\dag$ & $0.069^\dag$ & $\text{-}0.543^\dag$ \\
         Smooth Grad & $\text{-}0.470^\dag$ & $\text{-}0.025$~~ & $\text{-}0.349^\dag$ \\
         LRP & $\text{-}0.602^\dag$ & $0.001$~~ & $\text{-}0.446^\dag$ \\
         Confidence & $\text{-}1.000^\dag$ & $\text{-}0.121^\dag$ & $\text{-}0.697^\dag$ \\
        \bottomrule
    \end{tabular}}
\caption{Spearman correlation between APEM values for each explanation method and the loss of the evaluated model ($\dag$ represents statistical significance with $\rho < 0.01$). The correlation of the confidence of the most probable label and the loss is also presented for comparison.% These correlations are taken for the correctly classified images, the misclassified ones, and the full set of images.
    }
    \label{tab:corr}
\end{table}

